Polylogarithmic Approximation for Robust s-t Path

The paper revisits the robust $s$-$t$ path problem, one of the most fundamental problems in robust optimization. In the problem, we are given a directed graph with $n$ vertices and $k$ distinct cost functions (scenarios) defined over edges, and aim to choose an $s$-$t$ path such that the total cost of the path is always provable no matter which scenario is realized. With the view of each cost function being associated with an agent, our goal is to find a common $s$-$t$ path minimizing the maximum objective among all agents, and thus create a fair solution for them. The problem is hard to approximate within $o(\log k)$ by any quasi-polynomial time algorithm unless $\mathrm{NP} \subseteq \mathrm{DTIME}(n^{\mathrm{poly}\log n})$, and the best approximation ratio known to date is $\widetilde{O}(\sqrt{n})$ which is based on the natural flow linear program. A longstanding open question is whether we can achieve a polylogarithmic approximation even when a quasi-polynomial running time is allowed. We give the first polylogarithmic approximation for robust $s$-$t$ path since the problem was proposed more than two decades ago. In particular, we introduce a $O(\log n \log k)$-approximate algorithm running in quasi-polynomial time. The algorithm is built on a novel linear program formulation for a decision-tree-type structure which enables us to get rid of the $\Omega(\max\{k,\sqrt{n}\})$ integrality gap of the natural flow LP. Further, we also consider some well-known graph classes, e.g., graphs with bounded treewidth, and show that the polylogarithmic approximation can be achieved polynomially on these graphs. We hope the new proposed techniques in the paper can offer new insights into the robust $s$-$t$ path problem and related problems in robust optimization.

==> 20-preliminaries.tex <==
\subsection{Problem Formulation}
% \ruilong{move to other places}

Given a directed graph $G:=(V, E)$ with a source $s$ and a sink $t$, the number of vertices and edges are designated as $n$ and $m$, respectively.
Without loss of generality, we assume that the source vertex $s$ has no incoming edge, and the sink vertex $t$ has no outgoing edge.
In addition, there are $k$ scenarios, each of which represents a realization of the arc costs. 
Each scenario is represented by an agent in the set $A:=\set{1,\ldots,k}$, where agent $i$ has an additive arc cost function $c_i: 2^{E}\to \R_{\geq 0}$.
A feasible solution is defined as an $s \tto t$ path $\cP$, and the cost of agent $i$ is evaluated as $c_i(\cP):=\sum_{e\in\cP} c_i(e)$.
We aim to minimize the maximum cost across all agents, i.e., to find an $s \tto t$ path $\cP$ such that $\max_{i\in[k]}c_i(\cP)$ is minimized.


